Improved List Decoding for Polar-Coded Probabilistic Shaping

A modified successive cancellation list (SCL) decoder is proposed for polar-coded probabilistic shaping. The decoder exploits the deterministic encoding rule for shaping bits to rule out candidate code words that the encoder would not generate. This provides error detection and decreases error rates compared to standard SCL decoding while at the same time reducing the length of the outer cyclic redundancy check code.

==> tikzlibrarydsp.code.tex <==

\usetikzlibrary{arrows,
	calc,
	positioning,
	decorations.markings,
	shapes,
	decorations}


\newcommand{\dsplinewidth}{0.25mm}           %
\newcommand{\dspblocklinewidth}{0.3mm}       %
\newcommand{\dspoperatordiameter}{4mm}       %
\newcommand{\dspoperatorlabelspacing}{2mm}   %
\newcommand{\dspnoderadius}{1mm}             %
\newcommand{\dspsquareblocksize}{8mm}        %
\newcommand{\dspfilterwidth}{14mm}           %


\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} %
	\pgfsetmiterjoin	 %
	\pgfsetbuttcap		 %
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}


\makeatletter


\pgfkeys{/tikz/dsp/label/.initial=above}

\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }

	  \foreach \x in {center, mid, mid west, mid east, base, base west, base east,
	  	north, north east, east, south east, south, south west, west, north west}{
	  	\inheritanchor[from={circle}]{\x}
	  }
	  \inheritanchorborder[from={circle}]

	  %
	  \backgroundpath
	  {
	    %
	    \pgfpathcircle{\centerpoint}{\radius}

	    %
	    %
	    #2
	  }

	  \anchor{text}
	  {
			\centerpoint
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima

	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}

	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}

	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima

	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}

	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}

	\pgfusepathqstroke
}

\pgfdeclareshape{dspshapesaturation}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		\pgfpathmoveto{\pgfpoint{0}{0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0}{-0.33\pgf@ya}}
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa}{0}}
		\pgfpathlineto{\pgfpoint{-0.33\pgf@xa}{0}}
		\pgfpathmoveto{\pgfpointadd{\southwest}{\pgfpoint{-0.33\pgf@xa}{-0.6\pgf@ya}}}
		\pgfpathlineto{\pgfpointadd{\southwest}{\pgfpoint{-0.5\pgf@xa}{-0.6\pgf@ya}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-0.5\pgf@xa}{-0.6\pgf@ya}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-0.33\pgf@xa}{-0.6\pgf@ya}}}
	}
}


\pgfdeclareshape{dspshapelowpass}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa} {-0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.33\pgf@xa} {0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.33\pgf@xa} {0.33\pgf@ya}}
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa} {-0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.\pgf@xa} {-0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.2\pgf@xa} {0.33\pgf@ya}}
	}
}


\pgfdeclareshape{dspshapebandpass}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa} {-0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.33\pgf@xa} {0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.33\pgf@xa} {0.33\pgf@ya}}
		\pgfpathmoveto{\pgfpoint{0.15\pgf@xa} {0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.1\pgf@xa} {-0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.1\pgf@xa} {-0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.15\pgf@xa} {0.33\pgf@ya}}
	}
}


\pgfdeclareshape{dspshapesinewave}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast

		\pgfpathmoveto{\pgfpoint{0}{0.33\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0}{-0.33\pgf@ya}}
		\pgfpathmoveto{\pgfpoint{0.33\pgf@xa}{0}}
		\pgfpathlineto{\pgfpoint{-0.33\pgf@xa}{0}}

		\pgfpathmoveto{\pgfpoint{0.3\pgf@xa}{0}}
		\pgfpathsine{\pgfpoint{-0.15\pgf@xa}{0.25\pgf@ya}}
		\pgfpathcosine{\pgfpoint{-0.15\pgf@xa}{-0.25\pgf@ya}}
		\pgfpathsine{\pgfpoint{-0.15\pgf@xa}{-0.25\pgf@ya}}
		\pgfpathcosine{\pgfpoint{-0.15\pgf@xa}{0.25\pgf@ya}}
	}
}


\pgfdeclareshape{dspshapepulse}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\foregroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast

		\pgfpathmoveto{\pgfpoint{0.3\pgf@xa}{0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.15\pgf@xa}{0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.15\pgf@xa}{-0.15\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.15\pgf@xa}{-0.15\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.15\pgf@xa}{0.2\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.3\pgf@xa}{0.2\pgf@ya}}
	}
}


\pgfdeclareshape{dspshapeadaptive}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\anchor{arrowstart}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\southwest
		\advance\pgf@x by -0.05\pgf@xa
		\advance\pgf@y by 0.3\pgf@ya
	}

	\anchor{arrowend}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		\advance\pgf@x by 0.05\pgf@xa
		\advance\pgf@y by -0.3\pgf@ya
	}

	\behindbackgroundpath
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y

		\southwest
		\advance\pgf@x by -0.05\pgf@xa
		\advance\pgf@y by 0.3\pgf@ya
		\pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}

		\northeast
		\advance\pgf@x by 0.05\pgf@xa
		\advance\pgf@y by -0.3\pgf@ya

		\pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
		\pgfsetarrowsend{latex}
		\pgfsetlinewidth{\dsplinewidth}
		\pgfsetroundcap
		\pgfusepath{stroke}
	}

	\beforebackgroundpath
	{
    	\pgfpathrectanglecorners
		{\pgfpointadd{\southwest}{\pgfpoint{\dspblocklinewidth}{\dspblocklinewidth}}}
		{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\dspblocklinewidth}{\dspblocklinewidth}}}}

		\color{white}
		\pgfusepath{fill}
	}


}


\pgfdeclareshape{dspshapefourpole}{

	\inheritsavedanchors[from={rectangle}]
	\inheritbackgroundpath[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\anchor{west top}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@ya=\pgf@y
		\pgf@process{\southwest}
		\advance\pgf@y by -0.85\pgf@ya
	}

	\anchor{west bottom}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@ya=\pgf@y
		\pgf@process{\southwest}
		\advance\pgf@y by -0.15\pgf@ya
	}

	\anchor{east top}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@ya=\pgf@y
		\pgf@process{\northeast}
		\advance\pgf@y by 0.15\pgf@ya
	}

	\anchor{east bottom}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@ya=\pgf@y
		\pgf@process{\northeast}
		\advance\pgf@y by 0.85\pgf@ya
	}
}


\pgfdeclareshape{dspshapemic}{

	\inheritsavedanchors[from={circle}]
	\inheritbackgroundpath[from={circle}]
	\inheritanchorborder[from={circle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}	{
		\inheritanchor[from={circle}]{\x}
	}


	\beforebackgroundpath{
	\pgfmathsetlength\pgf@xa{\radius}

	\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@xa}}
	\pgfpathlineto{\pgfpoint{\pgf@xa}{-\pgf@xa}}

	\pgfusepathqstroke
	}
}


\pgfdeclareshape{dspshapespeaker}{

	\inheritsavedanchors[from={rectangle}]
	\inheritanchorborder[from={rectangle}]
	\foreach \x in {center, mid, mid west, mid east, base, base west, base east,
		north, north east, east, south east, south, south west, west, north west}{
		\inheritanchor[from={rectangle}]{\x}
	}

	\anchor{speaker}
	{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast
		\advance\pgf@x by -\pgf@xa
		\advance\pgf@y by 0.5\pgf@ya
	}

	\backgroundpath{
		\pgfpointdiff{\northeast}{\southwest}
		\pgf@xc=\pgf@x \pgf@yc=\pgf@y

		\pgfpathmoveto{\northeast}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-\pgf@xc}{-0.5\pgf@yc}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-\pgf@xc}{1.5\pgf@yc}}}
		\pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{0}{1\pgf@yc}}}

		\pgfpathrectanglecorners{\southwest}{\northeast}

	}

}


\def\pgf@dec@dashon{5pt}
\def\pgf@dec@dashoff{5pt}
\pgfkeys{/pgf/decoration/.cd,
	/pgf/decoration/dash on/.store in=\pgf@dec@dashon,
	/pgf/decoration/dash off/.store in=\pgf@dec@dashoff
}
\pgfdeclaredecoration{aligned dash}{start}{
	\state{start}[width=0pt, next state=pre-corner,persistent precomputation={
		\pgfextract@process\pgffirstpoint{\pgfpointdecoratedinputsegmentfirst}%
		\pgfextract@process\pgfsecondpoint{\pgfpointdecoratedinputsegmentlast}%
		\pgfmathsetlengthmacro\pgf@dec@dashon{\pgf@dec@dashon}%
		\pgfmathsetlengthmacro\pgf@dec@dashoff{\pgf@dec@dashoff}%
		\pgfmathsetlengthmacro\pgf@dec@halfdash{\pgf@dec@dashon/2}%
	}]{}
	\state{pre-corner}[width=\pgfdecoratedinputsegmentlength, next state=post-corner, persistent precomputation={
		\pgfmathparse{int(ceil((\pgfdecoratedinputsegmentlength-\pgf@dec@dashon-\pgf@dec@dashoff)/(\pgf@dec@dashon+\pgf@dec@dashoff)))}%
		\let\pgf@n=\pgfmathresult
		\pgfmathsetlengthmacro\pgf@b%
		{\pgfdecoratedinputsegmentlength/(\pgf@n+1)-\pgf@dec@dashon}%
		\ifdim\pgf@b<\pgf@dec@dashoff\relax%
		\pgfmathparse{int(\pgf@n-1)}\let\pgf@n=\pgfmathresult%
		\pgfmathsetlengthmacro\pgf@b%
		{\pgfdecoratedinputsegmentlength/(\pgf@n+1)-\pgf@dec@dashon}%
		\fi%
		\pgfmathsetlengthmacro\pgf@b{\pgf@b+\pgf@dec@dashon}%
	}]{%
		\pgfmathloop
		\ifnum\pgfmathcounter>\pgf@n%
		\else%
		\pgfpathmoveto{\pgfpoint{\pgf@b*\pgfmathcounter-\pgf@dec@halfdash}{0pt}}%
		\pgfpathlineto{\pgfpoint{\pgf@b*\pgfmathcounter+\pgf@dec@halfdash}{0pt}}%
		\repeatpgfmathloop%
		\pgfpathmoveto%
		{\pgfpoint{\pgfdecoratedinputsegmentlength-\pgf@dec@halfdash}{0pt}}%
		\pgfpathlineto%
		{\pgfpointdecoratedinputsegmentlast}
	}
	\state{post-corner}[width=0pt, next state=pre-corner]{
		\pgfpathlineto{\pgfpoint{\pgf@dec@halfdash}{0pt}}%
	}
	\state{final}{
		\pgftransformreset%
		\pgfpathlineto{\pgfpointlineatdistance{\pgf@dec@halfdash}{\pgffirstpoint}{\pgfsecondpoint}}%
	}
}


\makeatother


\tikzset{aligned dash/.style=
	{
		decoration=
		{
			aligned dash,
			#1
		},
		decorate
	}
}



\tikzset{dspadder/.style=
	{
		shape=dspshapeadder,
		line cap=rect,
		line join=rect,
		line width=\dspblocklinewidth,
		minimum size=\dspoperatordiameter
	}
}


\tikzset{dspmultiplier/.style=
	{
		shape=dspshapecircle,
		line cap=rect
		,line join=rect,
		line width=\dspblocklinewidth,
		minimum size=\dspoperatordiameter
	}
}


\tikzset{dspmixer/.style=
	{
		shape=dspshapemixer,
		line cap=rect,
		line join=rect,
		line width=\dspblocklinewidth,
		minimum size=\dspoperatordiameter
	}
}


\tikzset{dspnodeopen/.style=
	{
		shape=dspshapecircle,
		line width=\dsplinewidth,
		minimum size=\dspnoderadius
	}
}


\tikzset{dspnodefull/.style=
	{
		shape=dspshapecirclefull,
		line width=\dsplinewidth,
		fill,
		minimum size=\dspnoderadius
	}
}

\tikzset{dspsquare/.style=
	{
		shape=rectangle,
		draw,
		align=center,
		text depth=0.3em,
		text height=1em,
		inner sep=0pt,
		line cap=round,
		line join=round,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dspfilter/.style=
	{
		shape=rectangle,
		draw,
		align=center,
		text depth=0.3em,
		text height=1em,
		inner sep=0pt,
		line cap=round,
		line join=round,
		line width=\dsplinewidth,
		minimum height=\dspsquareblocksize,
		minimum width=\dspfilterwidth
	}
}


\tikzset{dspgain/.style=
	{
		draw,
		isosceles triangle,
		isosceles triangle apex angle=60,
		minimum width = \dspsquareblocksize,
		inner sep = 0pt
	}
}


\tikzset{dspsaturate/.style=
	{
		draw,
		shape=dspshapesaturation,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dspsinewave/.style=
	{
		draw,
		shape=dspshapesinewave,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dsppulse/.style=
	{
		draw,
		shape=dspshapepulse,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dsplowpass/.style=
	{
		draw,
		shape=dspshapelowpass,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dspbandpass/.style=
	{
		draw,
		shape=dspshapebandpass,
		line width=\dspblocklinewidth,
		minimum size=\dspsquareblocksize
	}
}


\tikzset{dspadaptivefilter/.style=
	{
		draw,
		shape=dspshapeadaptive,
		line width=\dspblocklinewidth,
		minimum height = \dspsquareblocksize,
		minimum width=\dspfilterwidth
	}
}


\tikzset{dspsystem/.style=
	{
		draw,
		line width = 0.5*\dspblocklinewidth,
		inner sep = 10pt,
		aligned dash =
		{
		}
	}
}


\tikzset{dspmic/.style=
	{
		draw,
		shape = dspshapemic,
		line width = \dspblocklinewidth,
		minimum size = \dspoperatordiameter
	}
}


\tikzset{dspspeaker/.style=
	{
		draw,
		shape = dspshapespeaker,
		line width = \dspblocklinewidth,
	}
}


\tikzset{dspfourpole/.style=
	{
		draw,
		shape = dspshapefourpole,
		inner sep = 0cm,
		line width = \dspblocklinewidth,
		minimum size = 2.6*\dspsquareblocksize
	}
}



\tikzset{dspline/.style=
	{
		line width=\dsplinewidth
	},
	line cap=round,
	line join=round
}


\tikzset{dspconn/.style=
	{
		->,
		>=dsparrow,
		line width=\dsplinewidth
	},
	line cap=round,
	line join=round
}


\tikzset{dspflow/.style=
	{
		line width=\dsplinewidth,
		line cap=round,
		line join=round,
		decoration=
		{
			markings,
			mark=at position 0.5 with
			{
				\arrow{dsparrowmid}
			}
		},
		postaction={decorate}
	}
}


\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}
